Modeling Bottom-Up and Top-Down Attention with a Neurodynamic Model of V1

Previous studies suggested that lateral interactions of V1 cells are responsible, among other visual effects, of bottom-up visual attention (alternatively named visual salience or saliency). Our objective is to mimic these connections with a neurodynamic network of firing-rate neurons in order to predict visual attention. Early visual subcortical processes (i.e. retinal and thalamic) are functionally simulated. An implementation of the cortical magnification function is included to define the retinotopical projections towards V1, processing neuronal activity for each distinct view during scene observation. Novel computational definitions of top-down inhibition (in terms of inhibition of return and selection mechanisms), are also proposed to predict attention in Free-Viewing and Visual Search tasks. Results show that our model outpeforms other biologically-inpired models of saliency prediction while predicting visual saccade sequences with the same model. We also show how temporal and spatial characteristics of inhibition of return can improve prediction of saccades, as well as how distinct search strategies (in terms of feature-selective or category-specific inhibition) can predict attention at distinct image contexts.

==> header_elsevier.tex <==



\vspace*{0.2in}
\date{July 2019}
\begin{flushleft}
{\Large
\textbf\newline{Modeling Bottom-Up and Top-Down Attention with a Neurodynamic Model of V1} % 
}
\newline
% Insert author names, affiliations and corresponding author email (do not include titles, positions, or degrees).
\\
David Berga\textsuperscript{1,2*},
Xavier Otazu\textsuperscript{1,2}
\\
\bigskip
\textbf{1} Computer Vision Center, Universitat Aut\`onoma de Barcelona, Barcelona, Spain
\\
\textbf{2} Dept. of Computer Science, Universitat Aut\`onoma de Barcelona, Barcelona, Spain
\\
\bigskip

* Corresponding author: dberga@cvc.uab.es

\end{flushleft}

% Please keep the abstract below 300 words
\section*{Abstract}  %xo: retocar mes, posar resultats, ampliar ...

Previous studies in that line suggested that lateral interactions of V1 cells are responsible, among other visual effects, of bottom-up visual attention (alternatively named visual salience or saliency). Our objective is to mimic these connections in the visual system with a neurodynamic network of firing-rate neurons. Early subcortical processes (i.e. retinal and thalamic) are functionally simulated. An implementation of the cortical magnification function is included to define the retinotopical projections towards V1, processing neuronal activity for each distinct view during scene observation. Novel computational definitions of top-down inhibition (in terms of inhibition of return and selection mechanisms), are also proposed to predict attention in Free-Viewing and Visual Search conditions. Results show that our model outpeforms other biologically-inpired models of saliency prediction as well as to predict visual saccade sequences during free viewing. We also show how temporal and spatial characteristics of inhibition of return can improve prediction of saccades, as well as how distinct search strategies (in terms of feature-selective or category-specific inhibition) predict attention at distinct image contexts.


\linenumbers

%Title MODVIS:Proposing simulations of top-down and recurrent inhibition in visual attention
%Abstract MODVIS: We propose a unified model of the visual cortex able to predict, among other effects, top-down visual attention and saccadic eye movements. First, we simulate activations of early mechanisms of the visual system (RP, RGC, LGN) towards the visual cortex (V1) by processing digital images. Second, images are projected to a cortically-magnified space to reproduce foveation. Third, with a neurodynamic model of lateral interactions in V1, we can reproduce contrast enhancement mechanisms present in the visual system, abling the prediction of visual saliency, brightness and chromatic induction. Fourth, projections towards the SC will serve as targets of saccade programming (scanpaths). Accounting for the last cases, activations from V1 and SC will be integrated as inhibition of return mechanisms towards LIP/FEF and back to SC/V1. This recurrent inhibition process will vary predictions of visual scanpaths. Top-down inhibition from working memory and goal-directed selection mechanisms are also proposed to predict attention in Free-Viewing and Visual Search conditions


